Multi-task Adversarial Attacks against Black-box Model with Few-shot Queries

Current multi-task adversarial text attacks rely on abundant access to shared internal features and numerous queries, often limited to a single task type. As a result, these attacks are less effective against practical scenarios involving black-box feedback APIs, limited queries, or multiple task types. To bridge this gap, we propose \textbf{C}luster and \textbf{E}nsemble \textbf{M}ulti-task Text Adversarial \textbf{A}ttack (\textbf{CEMA}), an effective black-box attack that exploits the transferability of adversarial texts across different tasks. CEMA simplifies complex multi-task scenarios by using a \textit{deep-level substitute model} trained in a \textit{plug-and-play} manner for text classification, enabling attacks without mimicking the victim model. This approach requires only a few queries for training, converting multi-task attacks into classification attacks and allowing attacks across various tasks. CEMA generates multiple adversarial candidates using different text classification methods and selects the one that most effectively attacks substitute models. In experiments involving multi-task models with two, three, or six tasks--spanning classification, translation, summarization, and text-to-image generation--CEMA demonstrates significant attack success with as few as 100 queries. Furthermore, CEMA can target commercial APIs (e.g., Baidu and Google Translate), large language models (e.g., ChatGPT 4o), and image-generation models (e.g., Stable Diffusion V2), showcasing its versatility and effectiveness in real-world applications.

==> section/method.tex <==

\section{Method}
Our method, CEMA, follows these steps: 
\ding{182} \textbf{Representation Learning} (Section \ref{rl}): We convert auxiliary texts and their outputs from multiple tasks into vector representations. 
\ding{183} \textbf{Clustering for Labels} (Section \ref{cluster-pse-lab}): After determining the optimal number of clusters, we apply a clustering algorithm to the vector representations and assign cluster labels to each auxiliary text. 
\ding{184} \textbf{Training Substitute Models} (Section \ref{substitute-model}): We train substitute models $f^{\text{s}}$ using auxiliary texts and their corresponding cluster labels. 
\ding{185} \textbf{Generating Adversarial Candidates} (Section \ref{Can_Sample}): We apply various adversarial attack methods to the substitute model $f^{\text{s}}$ to generate multiple adversarial candidates. 
\ding{186} \textbf{Selecting Final Adversarial Example} (Section \ref{final_Sample}): By iterating steps \ding{182}, \ding{183}, and \ding{184}, we train multiple substitute models \(f_1^{\text{s}}, f_2^{\text{s}}, \dots, f_M^{\text{s}}\). The final adversarial example is the candidate that successfully attacks the most substitute models.
\subsection{Representation learning}\label{rl}
In a multi-task model, both the input text and output labels need to be appropriately vectorized to effectively capture the relevant information. 
Pre-trained models are extensively utilized in NLP for textual feature extraction~\citep{tabassum2020survey, han2021pre}.  Furthermore, concatenating multiple text representations allows for the simultaneous encoding of multiple texts~\citep{devlin2018bert}. Accordingly, we leverage a pre-trained model to vectorize both the input text and output labels, generating their respective embeddings. These embeddings are subsequently concatenated to form a unified representation that captures the information from both the input text and the output labels.
As outlined in Algorithm \ref{alg_substitute} (lines 1-5), we first query the multi-task model $f_v$ to retrieve output texts for each task. Auxiliary texts, along with corresponding outputs, are vectorized using the pre-trained model $f_{\text{pre}}$ to extract features for clustering. The multi-task model $f_v$ handles tasks ${A,B,\dots,N}$, while the attacker has access to a small set of auxiliary texts $\boldsymbol{X}$, sampled from the same distribution as the victim texts. For each auxiliary text $x_i$ in $\boldsymbol{X}$, we query $f_v$ to obtain outputs $y_i^A, y_i^B, \dots, y_i^N$. The pre-trained model $f_{\text{pre}}$ then vectorizes $x_i$ and its outputs, producing vectors $\{\boldsymbol{E}_{x_i}, \boldsymbol{E}_{y_i^A}, \dots, \boldsymbol{E}_{y_i^N}\}$, which are concatenated to form the final vector $\boldsymbol{E}_i$, representing $x_i$ and its outputs. Thus, $\boldsymbol{E}_i$ is defined as:
\begin{equation}
\begin{aligned}
\boldsymbol{E}_{x_i} &= f_{\text{pre}}(x_i), \quad
\boldsymbol{E}_{y_i^J} = f_{\text{pre}}(y_i^J), \\
\boldsymbol{E}_{i} &= \text{Concat}(\boldsymbol{E}_{x_i},\boldsymbol{E}_{y_i^A},\dots,\boldsymbol{E}_{y_i^N}),
\end{aligned}
\end{equation}
where the $Concat$ indicates the concatenation of $\{\boldsymbol{E}_{x_i},\boldsymbol{E}_{y_i^A},\dots,\boldsymbol{E}_{y_i^N}\}$.


\subsection{Cluster Number and Cluster Labels}\label{cluster-pse-lab}


In Section \ref{rl}, we obtain the representations for each text input and output. We then perform a clustering analysis on these representations, with the number of clusters being a crucial parameter. Before clustering, we determine the optimal number of clusters by selecting the value that maximizes strong discriminative capability for each cluster group. 
When the number of clusters is $2$, the two clusters can be interpreted as class $C_A$ and $\overline{C_A}$.~\citep{boongoen2018cluster}. Therefore, we set the number of clusters to $2$.



    
\subsection{Substitute Model Training }\label{substitute-model}

Once the cluster labels are obtained, we employ the auxiliary texts paired with their respective cluster labels to train a substitute model. This approach effectively converts the multi-task text adversarial attack scenario into a conventional text classification adversarial attack scenario. The substitute model $f^{\text{s}}$ is trained with the auxiliary texts serving as input data and the cluster labels as the corresponding output labels. The process is shown in lines 10-12 of Algorithm \ref{alg_substitute}.
More details about the substitute model architecture and substitute model training are presented in Appendix \ref{substitute-model-architecture}.

\subsection{Candidate Adversarial Example Generation}\label{Can_Sample}



Once the substitute model is generated, we apply several adversarial text attack methods to $f^{\text{s}}$, producing multiple adversarial examples. We then define criteria to select the final adversarial example from the generated candidates. In this section, we first explain the importance of generating multiple adversarial candidate examples. Let $m$ adversarial attack methods generate $m$ adversarial examples on the substitute model $f_1^{\text{\text{s}}}$. Denote these adversarial examples as $x_i^{*1}, x_i^{*2}, \dots, x_i^{*m}$, with corresponding probabilities of successful attacks on the victim model denoted as $p_i^{*1}, p_i^{*2}, \dots, p_i^{*m}$. As $m$ increases, the probability, $p_m^s$, that at least one of these adversarial examples successfully attacks the victim model also increases. This is formalized in Theorem \ref{max_prob2}.
\begin{theorem}\label{max_prob2}
$p^s_m$ is the probability that at least one of these adversarial examples successfully attacks the victim model with $m$ candidate adversarial examples, formally：
\end{theorem}
\textit{Proof.} Please refer to Appendix~\ref{proof_max_prob2} for details.




\subsubsection{Transferability-Oriented Adversarial Example Selection}\label{final_Sample}
In Section \ref{Can_Sample}, we demonstrate that generating additional adversarial candidate examples increases the likelihood of finding a successful adversarial example, which can then effectively attack the victim model.
This section focuses on the process of selecting the most likely successful adversarial example from the generated candidates. We explore the criteria and methods used to identify the most effective example.

We first select the adversarial candidate with the highest transferability as the final example. To evaluate transferability, we train multiple substitute models and count the number of successful attacks against them. Ultimately, we choose the adversarial candidate that successfully attacks the most substitute models as the final adversarial example. 
The detailed steps are presented as follows:
\ding{182} \textbf{Training Multiple Substitute Models:}
We randomly sample 80\% of the $100$ auxiliary text-cluster label pairs to form the training set for a new substitute model. This process is repeated $w$ times, yielding $w$ substitute models, denoted as $f_1^{\text{s}}, f_2^{\text{s}}, \dots, f_w^{\text{s}}$.
\ding{183} \textbf{Calculating the Transferability Score:}
For each victim text \(x_k\), we generate \(m\) adversarial candidate examples, denoted as \(\{x_k^{*1}, x_k^{*2}, \dots, x_k^{*m}\}\). The transferability score for \(x_k^{*j}\) is calculated as follows:

\begin{equation}
\begin{aligned}
I_{k i j} &= \left\{
\begin{array}{cc}
1, & f_i^{\text{s}}\left(x^{* j}_k\right) \neq f_i^{\text{s}}(x_k); \\
0, & f_i^{\text{s}}\left(x^{* j}_k\right) = f_i^{\text{s}}(x_k);
\end{array}
\right. \\
I_{k j} &= \sum_{i=1}^w I_{k i j}, \quad
j = \arg\max_j\ I_{k j}.
\end{aligned}
\end{equation}

where $f_i^{\text{s}}\left(x^{* j}_k\right)$ represents the output label of $x^{* j}_k$ is produced by the substitute model $f_i^{\text{s}}$. Similarly, $f_i^{\text{s}}(x_k)$ is the output label of $x_k$ generated by the same model. If $f_i^{\text{s}}\left(x^{* j}_k\right) \neq f_i^{\text{s}}(x_k)$, then $x^{* j}_k$ successfully attacks the substitute model $f_i^{\text{s}}$. Therefore, $I_{k j}$ measures the number of substitute models that $x^{* j}_k$ successfully attacks. The adversarial example that successfully attacks the largest number of substitute models is then selected as the final adversarial example. In other words, adversarial examples capable of attacking multiple substitute models demonstrate greater transferability and higher probability of successfully attacking the victim model $f_v$.

==> section/observations_and_motivations.tex <==
\section{Observations and Motivations}
\label{sec:observations}
NO YET

==> section/preliminaries_and_background.tex <==
\section{Preliminary}















\textbf{Transferability and multi-task learning.}
Transferability refers to the ability of adversarial examples, crafted for one model, to successfully attack other models~\citep{zhang2020two,papernot2017practical,mahmood2021beware,zhou2020dast}. 
Multi-task learning trains multiple related tasks together, enabling knowledge sharing and improving generalization~\cite{cai2025multimodal,pu2025integrating}.

\noindent\textbf{Auxiliary data.}
 Auxiliary data refers to additional information used to assist in generating adversarial examples. This data, which is not part of the original input, helps attackers better understand the target model's behavior or generate more effective adversarial inputs. For instance,  auxiliary data might include outputs from the victim model~\cite{chen2024reversible, papernot2017practical}.







==> section/related_work.tex <==
\section{Related Work}
In appendix


